THRONE: An Object-based Hallucination Benchmark for the Free-form Generations of Large Vision-Language Models

Mitigating hallucinations in large vision-language models (LVLMs) remains an open problem. Recent benchmarks do not address hallucinations in open-ended free-form responses, which we term "Type I hallucinations". Instead, they focus on hallucinations responding to very specific question formats -- typically a multiple-choice response regarding a particular object or attribute -- which we term "Type II hallucinations". Additionally, such benchmarks often require external API calls to models which are subject to change. In practice, we observe that a reduction in Type II hallucinations does not lead to a reduction in Type I hallucinations but rather that the two forms of hallucinations are often anti-correlated. To address this, we propose THRONE, a novel object-based automatic framework for quantitatively evaluating Type I hallucinations in LVLM free-form outputs. We use public language models (LMs) to identify hallucinations in LVLM responses and compute informative metrics. By evaluating a large selection of recent LVLMs using public datasets, we show that an improvement in existing metrics do not lead to a reduction in Type I hallucinations, and that established benchmarks for measuring Type I hallucinations are incomplete. Finally, we provide a simple and effective data augmentation method to reduce Type I and Type II hallucinations as a strong baseline. Code is now available at https://github.com/amazon-science/THRONE .

==> assets/tables/POPE_results.tex <==
\begin{table}[h!]
\scriptsize
\begin{adjustbox}{width=\linewidth}
\centering
\setlength\tabcolsep{2pt}
\begin{tabular}{@{}l|ccc|ccc|ccc@{}}
\toprule
                               &\multicolumn{3}{c|}{Precision}                    & \multicolumn{3}{c|}{Recall}                      & \multicolumn{3}{c}{F1 Score}                     \\
\multirow{-2}{*}{Method}       & POPE & Ex. POPE & $\Delta$                       & POPE & Ex. POPE & $\Delta$                       & POPE & Ex. POPE & $\Delta$                       \\ \midrule
LLaMA-Adapter-LORA-BIAS-7B-v21 & 62.2 & 27.1     & {\color[HTML]{FF0000} (-35.1)} & 96.0 & 90.3     & {\color[HTML]{FF0000} (-5.8)}  & 75.4 & 41.7     & {\color[HTML]{FF0000} (-33.7)} \\
LLaMA-Adapter-LORA-BIAS-7B     & 59.8 & 20.3     & {\color[HTML]{FF0000} (-39.4)} & 93.0 & 91.1     & {\color[HTML]{FF0000} (-1.9)}  & 72.5 & 33.3     & {\color[HTML]{FF0000} (-39.3)} \\
LRV-Instruction-V2             & 71.4 & 3.8      & {\color[HTML]{FF0000} (-67.6)} & 89.5 & 100.0    & {\color[HTML]{009901} 10.5}    & 79.2 & 7.3      & {\color[HTML]{FF0000} (-71.9)} \\
OTTER-Image-MPT7B              & 78.5 & 10.6     & {\color[HTML]{FF0000} (-67.8)} & 88.7 & 96.7     & {\color[HTML]{009901} 7.9}     & 83.1 & 19.1     & {\color[HTML]{FF0000} (-64.0)} \\
Qwen-VL-Chat                   & 88.8 & 73.1     & {\color[HTML]{FF0000} (-15.8)} & 84.1 & 83.6     & {\color[HTML]{FF0000} (-0.5)}  & 86.3 & 78.0     & {\color[HTML]{FF0000} (-8.3)}  \\
instructblip-vicuna-7b         & 84.1 & 51.4     & {\color[HTML]{FF0000} (-32.7)} & 87.1 & 87.5     & {\color[HTML]{009901} 0.4}     & 85.4 & 64.8     & {\color[HTML]{FF0000} (-20.6)} \\
llava-v1.3-7b-lora             & 58.8 & 9.4      & {\color[HTML]{FF0000} (-49.4)} & 98.5 & 98.5     & 0.0                            & 73.5 & 17.1     & {\color[HTML]{FF0000} (-56.4)} \\
llava-v1.5-7b                  & 82.5 & 58.7     & {\color[HTML]{FF0000} (-23.8)} & 90.7 & 85.7     & {\color[HTML]{FF0000} (-5.0)}  & 86.3 & 69.7     & {\color[HTML]{FF0000} (-16.6)} \\
minigpt4-vicuna-7b-v0          & 52.3 & 6.8      & {\color[HTML]{FF0000} (-45.4)} & 96.4 & 85.2     & {\color[HTML]{FF0000} (-11.2)} & 67.8 & 12.6     & {\color[HTML]{FF0000} (-55.1)} \\
minigpt4v2-llama2-7b-chat      & 77.3 & 34.2     & {\color[HTML]{FF0000} (-43.1)} & 93.5 & 94.2     & {\color[HTML]{009901} 0.7}     & 84.5 & 50.2     & {\color[HTML]{FF0000} (-34.2)} \\
mplug-owl-llama-7b             & 53.7 & 9.1      & {\color[HTML]{FF0000} (-44.6)} & 98.9 & 97.5     & {\color[HTML]{FF0000} (-1.4)}  & 69.6 & 16.7     & {\color[HTML]{FF0000} (-52.9)} \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{POPE does not analyze Type II hallucinations across all categories for each image.
We find extending POPE to an exhaustive analysis leads to a dramatic reduction in performance across all models, demonstrating POPE severely underestimates Type II hallucinations in LVLMs.
}\label{tab:results_pope}
\end{table}

==> assets/tables/POPE_results_norecall.tex <==
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{l|ccc|ccc}
\toprule
                                               &\multicolumn{3}{c|}{Precision}                    & \multicolumn{3}{c}{F1 Score}                     \\
\multirow{-2}{*}{Method}                       & POPE & Ex. POPE & $\Delta$                       & POPE & Ex. POPE & $\Delta$                       \\ \midrule
LLaMA-Adapter-v2~\cite{gao2023llamaadapter}    & 59.8 & 20.3     & {\color[HTML]{FF0000} (-39.4)} & 72.5 & 33.3     & {\color[HTML]{FF0000} (-39.3)} \\
LLaMA-Adapter-v2.1~\cite{gao2023llamaadapter}  & 62.2 & 27.1     & {\color[HTML]{FF0000} (-35.1)} & 75.4 & 41.7     & {\color[HTML]{FF0000} (-33.7)} \\
InstructBLIP~\cite{dai2023instructblip}        & 84.1 & 51.4     & {\color[HTML]{FF0000} (-32.7)} & 85.4 & 64.8     & {\color[HTML]{FF0000} (-20.6)} \\
Otter-Image~\cite{li2023otter}                 & 78.5 & 10.6     & {\color[HTML]{FF0000} (-67.8)} & 83.1 & 19.1     & {\color[HTML]{FF0000} (-64.0)} \\
MiniGPT4~\cite{zhu2023minigpt}                 & 52.3 & 6.8      & {\color[HTML]{FF0000} (-45.4)} & 67.8 & 12.6     & {\color[HTML]{FF0000} (-55.1)} \\
MiniGPT-v2~\cite{chen2023minigpt2}             & 77.3 & 34.2     & {\color[HTML]{FF0000} (-43.1)} & 84.5 & 50.2     & {\color[HTML]{FF0000} (-34.2)} \\
Qwen-VL-Chat~\cite{Qwen-VL}                    & 88.8 & 73.1     & {\color[HTML]{FF0000} (-15.8)} & 86.3 & 78.0     & {\color[HTML]{FF0000} (-8.3)}  \\
mPLUG-Owl~\cite{ye2023mplug}                   & 53.7 & 9.1      & {\color[HTML]{FF0000} (-44.6)} & 69.6 & 16.7     & {\color[HTML]{FF0000} (-52.9)} \\
LRV-Instruction-v2~\cite{liu2023aligning}      & 71.4 & 3.8      & {\color[HTML]{FF0000} (-67.6)} & 79.2 & 7.3      & {\color[HTML]{FF0000} (-71.9)} \\
LLaVA-v1.3*~\cite{liu2023visual}               & 58.8 & 9.4      & {\color[HTML]{FF0000} (-49.4)} & 73.5 & 17.1     & {\color[HTML]{FF0000} (-56.4)} \\
LLaVA-v1.5~\cite{liu2023improved}              & 82.5 & 58.7     & {\color[HTML]{FF0000} (-23.8)} & 86.3 & 69.7     & {\color[HTML]{FF0000} (-16.6)} \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{POPE does not query every category of interest for Type II hallucinations.
Extending POPE to an exhaustive analysis on all COCO leads to a dramatic reduction in performance across all models,
demonstrating the fragility of POPE to the sampling mechanism. By under-sampling negative classes, POPE severely underestimates Type II hallucinations in LVLMs.
}\label{tab:results_pope}


% \begin{table}[h!]
% \scriptsize
% \begin{adjustbox}{width=\linewidth}
% \centering
% \setlength\tabcolsep{2pt}


% \end{table}

==> assets/tables/benchmark_POPE_results.tex <==
% ==================================================
\begin{table*}[t]
\begin{minipage}[!ht]{.58\linewidth}
\scriptsize
% \begin{adjustbox}{width=\columnwidth}
\centering
\setlength\tabcolsep{2pt}
\input{assets/tables/benchmark_results.tex}
% \end{adjustbox}
\end{minipage}
% ==================================================
\hfill
\begin{minipage}[!ht]{.40\linewidth}
\scriptsize
\setlength\tabcolsep{2pt}
\input{assets/tables/POPE_results_norecall.tex}
\end{minipage}
\vspace{-0.3cm}
\end{table*}

==> assets/tables/benchmark_results.tex <==
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{l|l|c|cccc|ccc>{\columncolor[HTML]{EFEFEF}}c}
\toprule
% \setlength\fboxsep{-10.0pt}
Method                                        & LLM                                     & $L$ & $P_\textsc{ALL}$                     & $R_\textsc{ALL}$                     & $F^1_{\textsc{ALL}}$                 & $F^{0.5}_{\textsc{ALL}}$             & $P_\textsc{CLS}$                     & $R_\textsc{CLS}$                     & $F^1_{\textsc{CLS}}$                 & $F^{0.5}_{\textsc{CLS}}$             \\ \midrule
LLaMA-Adapter-v2~\cite{gao2023llamaadapter}   & Llama1-7b~\cite{touvron2023llama}       & 514 & 63.6                                 & 73.3                                 & 68.1                                 & 65.3                                 & 68.2                                 & 70.6                                 & 69.4                                 & 68.7                                 \\
LLaMA-Adapter-v2.1~\cite{gao2023llamaadapter} & Llama1-7b~\cite{touvron2023llama}       & 512 & 63.8                                 & 73.7                                 & 68.4                                 & 65.5                                 & 67.4                                 & 71.2                                 & 69.3                                 & 68.1                                 \\
InstructBLIP~\cite{dai2023instructblip}       & Vicuna-v1.1-7b~\cite{chiang2023vicuna}  & 525 & 70.8                                 & {\color[HTML]{FF0000} \textit{74.3}} & {\color[HTML]{FF0000} \textit{72.5}} & 71.5                                 & 77.2                                 & {\color[HTML]{FF0000} \textit{71.9}} & {\color[HTML]{FF0000} \textit{74.5}} & 76.1                                 \\
Otter-Image~\cite{li2023otter}                & MPT-7b~\cite{mosaicml2023mpt}           & 257 & 33.0                                 & 31.2                                 & 32.1                                 & 32.7                                 & 25.2                                 & 16.9                                 & 20.2                                 & 22.9                                 \\
MiniGPT4~\cite{zhu2023minigpt}                & Vicuna-v0-7b~\cite{chiang2023vicuna}    & 473 & {\color[HTML]{FF0000} \textit{81.7}} & 59.8                                 & 69.0                                 & 76.1                                 & {\color[HTML]{0432FF} \textbf{79.9}} & 61.8                                 & 69.7                                 & 75.5                                 \\
MiniGPT-v2~\cite{chen2023minigpt2}            & Llama2-7b-chat~\cite{touvron2023llama2} & 381 & 79.0                                 & 66.6                                 & 72.3                                 & {\color[HTML]{FF0000} \textit{76.2}} & 77.6                                 & 67.0                                 & 71.9                                 & 75.2                                 \\
Qwen-VL-Chat~\cite{Qwen-VL}                   & Qwen-7b~\cite{bai2023qwen}              & 524 & 74.7                                 & {\color[HTML]{0432FF} \textbf{77.2}} & {\color[HTML]{0432FF} \textbf{75.9}} & 75.2                                 & 78.0                                 & {\color[HTML]{0432FF} \textbf{76.1}} & {\color[HTML]{0432FF} \textbf{77.0}} & {\color[HTML]{0432FF} \textbf{77.6}} \\
mPLUG-Owl~\cite{ye2023mplug}                  & Llama1-7b~\cite{touvron2023llama}       & 555 & 55.5                                 & 71.9                                 & 62.6                                 & 58.1                                 & 66.3                                 & 68.3                                 & 67.3                                 & 66.7                                 \\
LRV-Instruction-v2~\cite{liu2023aligning}     & Llama1-7b~\cite{touvron2023llama}       & 103 & {\color[HTML]{0432FF} \textbf{82.0}} & 56.7                                 & 67.0                                 & 75.3                                 & {\color[HTML]{FF0000} \textit{78.4}} & 58.8                                 & 67.2                                 & 73.5                                 \\
LLaVA-v1.3*~\cite{liu2023visual}              & Vicuna-v1.3-7b~\cite{chiang2023vicuna}  & 532 & 80.5                                 & 65.2                                 & 72.1                                 & {\color[HTML]{0432FF} \textbf{76.9}} & {\color[HTML]{0432FF} \textbf{79.9}} & 65.3                                 & 71.9                                 & {\color[HTML]{FF0000} \textit{76.5}} \\
LLaVA-v1.5~\cite{liu2023improved}             & Vicuna-v1.5-7b~\cite{chiang2023vicuna}  & 509 & 68.1                                 & 61.0                                 & 64.4                                 & 66.6                                 & 69.9                                 & 56.4                                 & 62.5                                 & 66.8                                 \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Evaluation results for a selection of instruction-tuned LVLMs on \throne with COCO.
We select $F^{0.5}_{\textsc{CLS}}$ as the principal metric for evaluation in our benchmark to balance across classes and to prioritize precision (which reflects the extent of hallucination) over recall.
{\color[HTML]{0432FF} \textbf{blue}} and {\color[HTML]{FF0000} \textit{red}} denote best and second-best performance, respectively.
*Our implementation using official code to enable fair comparison. $L$ corresponds to the median response length (measured in  $\#$ of characters).
\yoni{What is the message we should have for Table 1? It has a lot of great data we can use to drive a message, but we should re-think how to highlight/organize this data} }\label{tab:results_main}


% \begin{table*}[t]
% \centering
% \scriptsize
% \setlength\tabcolsep{3pt}

% \end{table*}


==> assets/tables/sampling_results.tex <==
\begin{table}[t]
\centering
\scriptsize
\begin{adjustbox}{width=\linewidth}
\setlength\tabcolsep{2pt}
\begin{tabular}{cccccccccccc}
    \toprule
    \rotatebox{75}{Method}           & \rotatebox{75}{LLaMA-Adapter-v2} & \rotatebox{75}{LLaMA-Adapter-v2.1} & \rotatebox{75}{InstructBLIP}  & \rotatebox{75}{Otter-Image}    & \rotatebox{75}{MiniGPT4}      & \rotatebox{75}{MiniGPT-v2}     & \rotatebox{75}{Qwen-VL-Chat}  & \rotatebox{75}{mPLUG-Owl}      & \rotatebox{75}{LRV-Instruction-V2} & \rotatebox{75}{LLaVA-v1.3-7b*} & \rotatebox{75}{LLaVA-v1.5-7b}  \\ \midrule
    \multicolumn{1}{c|}{Full (Ours)} & 68.7                             & 68.1                               & 76.1                          & 22.9                           & 75.5                          & 75.2                           & 77.6                          & 66.7                           & 73.5                               & 76.5                           & 66.8                           \\
    \multicolumn{1}{c|}{POPE}        & 84.4                             & 85.4                               & 84.9                          & 45.9                           & 83.0                          & 86.6                           & 87.3                          & 81.4                           & 79.4                               & 83.7                           & 81.4                           \\
    \multicolumn{1}{c|}{$\Delta$}    & {\color[HTML]{FF0000} (-15.7)}   & {\color[HTML]{FF0000} (-17.2)}     & {\color[HTML]{FF0000} (-8.8)} & {\color[HTML]{FF0000} (-23.0)} & {\color[HTML]{FF0000} (-7.5)} & {\color[HTML]{FF0000} (-11.4)} & {\color[HTML]{FF0000} (-9.7)} & {\color[HTML]{FF0000} (-14.7)} & {\color[HTML]{FF0000} (-5.9)}      & {\color[HTML]{FF0000} (-7.2)}  & {\color[HTML]{FF0000} (-14.6)} \\ \bottomrule
    \end{tabular}
\end{adjustbox}
\caption{\TODO{Move to supplementary}
}\label{tab:results_sampling}
\end{table}

==> sec/08-limit.tex <==

\cvprsection{Limitations}\label{sec:limit}

==> supplementary_material/preamble.tex <==
%
% --- inline annotations
%
\usepackage{booktabs}
\usepackage[table,xcdraw,dvipsnames]{xcolor}
\usepackage{multirow}
\usepackage{lipsum}
\usepackage{adjustbox}
\usepackage{colortbl}
\usepackage{amssymb}
\usepackage{pifont}
% \usepackage[pagebackref,breaklinks,colorlinks]{hyperref}
% \usepackage[numbers,sort]{natbib}
% \usepackage[dvipsnames]{xcolor}
% \linespread{2.0}
\usepackage{xspace}

\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO:\@ #1]}}
\newcommand{\best}[1]{{\color[HTML]{3531FF}{\textbf{#1}}}}
\newcommand{\sbest}[1]{{\color[HTML]{FE0000}{\textit{#1}}}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

\newcommand{\prannay}[1]{{\textcolor{red}{Prannay: #1} }}
\newcommand{\zhizhong}[1]{{\textcolor{blue}{Zhizhong: #1} }}
\newcommand{\hao}[1]{{\textcolor{magenta}{Hao: #1} }}
\newcommand{\yoni}[1]{{\textcolor{olive}{Yoni: #1} }}
\newcommand{\redact}[1]{{\textcolor{red}{Removing: #1} }}
\newcommand{\throne}{\textsc{THR\={O}NE}\xspace}

% % uncomment to blank all author comments
% \renewcommand{\prannay}[1]{}
% \renewcommand{\zhizhong}[1]{}
% \renewcommand{\hao}[1]{}
% \renewcommand{\yoni}[1]{}


\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}
\newcommand{\xmark}{\ding{55}}%
\newcommand{\texttts}[1]{\texttt{\footnotesize #1}}

==> supplementary_material/sm_sec/01-model_details.tex <==
\cvprsection{Evaluated LVLM Details}\label{smsec:model_details}
In this section, we briefly outline details in the LVLMs we evaluate with \throne, such as design choices and training data.

\paragraph*{LLaMA-Adapter-v2}~\cite{gao2023llamaadapter} \\
\begin{itemize}
    \item LLM:\@ LLaMA-v1-7b~\cite{touvron2023llama}
    \item Image Encoder: CLIP ViT-L/14~\cite{radford2021learning}
    \item Vision-Language Connector: Linear projection, learnt visual queries and additional vision transformer blocks 
    \item Pretraining Data:
    LAION-400M~\cite{schuhmann2021laion},
    COYO-700M~\cite{kakaobrain2022coyo-700m},
    MMC4~\cite{zhu2023multimodal},
    SBU~\cite{NIPS2011_5dd9db5e},
    CC3M~\cite{sharma2018conceptual},
    and COCO Captions~\cite{fang2015captions}
    \item Finetuning Data:
    GPT4LLM~\cite{peng2023instruction} and
    LLaVA~\cite{liu2023visual}
\end{itemize}

\paragraph*{LLaMA-Adapter-v2.1}~\cite{gao2023llamaadapter} \\
Same as LLaMA-Adapter-v2 with one modification.
\begin{itemize}
    \item Finetuning Data:
    GPT4LLM~\cite{peng2023instruction},
    LLaVA~\cite{liu2023visual} \emph{and
    VQAv2}~\cite{antol2015vqa}
\end{itemize}

\paragraph*{InstructBLIP}~\cite{dai2023instructblip} \\
\begin{itemize}
    \item LLM:\@ Vicuna-v1.1-7b~\cite{chiang2023vicuna}
    \item Image Encoder: EVA ViT-g/14~\cite{fang2023eva}
    \item Visual-Language Connector: Querying Transformer (Q-Former)
    \item Pretraining Data:
    LAION400M~\cite{schuhmann2021laion},
    CC3M~\cite{sharma2018conceptual},
    CC12M~\cite{changpinyo2021conceptual},
    Visual Genome~\cite{krishna2017visual}
    and COCO Captions~\cite{fang2015captions}
    \item Finetuning Data:
    COCO Captions~\cite{fang2015captions},
    TextCaps~\cite{sidorov2019textcaps},
    VQAv2~\cite{antol2015vqa},
    OKVQA~\cite{okvqa},
    A-OKVQA~\cite{AOKVQA},
    OCR-VQA~\cite{8978122} and
    LLaVA~\cite{liu2023visual}
\end{itemize}

\paragraph*{Otter-Image}~\cite{li2023otter} \\
\begin{itemize}
    \item LLM:\@ MPT-7b~\cite{mosaicml2023mpt} (initialized from OpenFlamingo weights~\cite{anas_awadalla_2023_7733589})
    \item Image Encoder: CLIP ViT-L/14~\cite{radford2021learning}
    \item Visual-Language Connector: Cross-attention modules between visual and language features
    \item Pretraining Data:
    MMC4~\cite{zhu2023multimodal},
    LAION-2B-en~\cite{schuhmann2022laion}
    and synthetic data from ChatGPT~\cite{openai2023chatgpt} 
    \item Finetuning Data: MIMIC-IT~\cite{li2023otter}
\end{itemize}

\paragraph*{MiniGPT-4}~\cite{zhu2023minigpt} \\
\begin{itemize}
    \item LLM:\@ Vicuna-v0-7b~\cite{chiang2023vicuna}
    \item Image Encoder: EVA ViT-g/14~\cite{fang2023eva}
    \item Vision-Language Connector: Linear projection and Q-Former (initialized and frozen from BLIP-2~\cite{li2023blip2})
    \item Pretraining Data:
    CC3M~\cite{sharma2018conceptual},
    CC12M~\cite{changpinyo2021conceptual},
    SBU~\cite{NIPS2011_5dd9db5e} and
    LAION-400M~\cite{schuhmann2021laion}
    \item Finetuning Data:
    Synthetic data using ChatGPT~\cite{openai2023chatgpt}
    and a sample of CC3M/CC12M images~\cite{changpinyo2021conceptual,sharma2018conceptual}
\end{itemize}

\paragraph*{MiniGPT-v2}~\cite{chen2023minigpt2} \\
\begin{itemize}
    \item LLM:\@ Llama2-7b-chat~\cite{touvron2023llama2}
    \item Image Encoder: EVA ViT-g/14~\cite{fang2023eva}
    \item Vision-Language Connector: Linear projection
    \item Pretraining Data:
    GRiT-20M~\cite{peng2023kosmos2},
    COCO Captions~\cite{fang2015captions},
    TextCaps~\cite{sidorov2019textcaps},
    RefCOCO/+/g~\cite{kazemzadeh2014referitgame,mao2016generation},
    Visual Genome~\cite{krishna2017visual},
    GQA~\cite{hudson2019gqa},
    VQAv2~\cite{antol2015vqa},
    OKVQA~\cite{okvqa},
    A-OKVQA~\cite{AOKVQA} and
    OCR-VQA~\cite{8978122}
    \item Finetuning Data:
    COCO Captions~\cite{fang2015captions},
    TextCaps~\cite{sidorov2019textcaps},
    RefCOCO/+/g~\cite{kazemzadeh2014referitgame,mao2016generation},
    Visual Genome~\cite{krishna2017visual},
    GQA~\cite{hudson2019gqa},
    VQAv2~\cite{antol2015vqa},
    OKVQA~\cite{okvqa},
    A-OKVQA~\cite{AOKVQA},
    LLaVA~\cite{liu2023visual},
    Flickr30k~\cite{plummer2015flickr30k} and
    LLaVA~\cite{liu2023visual}
\end{itemize}

\paragraph*{Qwen-VL-Chat}~\cite{Qwen-VL} \\
\begin{itemize}
    \item LLM:\@ Qwen-LM~\cite{bai2023qwen}
    \item Image Encoder: OpenCLIP ViT-g~\cite{ilharco_gabriel_2021_5143773}
    \item Vision-Language Connector: Single cross-attention block between image features and learnt visual queries 
    \item Pretraining Data:
    LAION-2B-en~\cite{schuhmann2022laion},
    COYO-700M~\cite{kakaobrain2022coyo-700m},
    CC3M~\cite{sharma2018conceptual},
    CC12M~\cite{changpinyo2021conceptual},
    SBU~\cite{NIPS2011_5dd9db5e},
    COCO Caption~\cite{fang2015captions}
    and DataComp~\cite{gadre2023datacomp}
    \item Finetuning Data:
    LAION-2B-en/zh~\cite{schuhmann2022laion},
    COYO-700M~\cite{kakaobrain2022coyo-700m},
    CC3M~\cite{sharma2018conceptual},
    CC12M~\cite{changpinyo2021conceptual},
    SBU~\cite{NIPS2011_5dd9db5e},
    DataComp~\cite{gadre2023datacomp},
    COCO Caption~\cite{fang2015captions},
    GQA~\cite{hudson2019gqa},
    Visual Genome~\cite{krishna2017visual},
    VQAv2~\cite{antol2015vqa},
    DVQA~\cite{kafle2018dvqa},
    OCR-VQA~\cite{8978122},
    DocVQA~\cite{mathew2021docvqa},
    TextVQA~\cite{singh2019towards},
    ChartQA~\cite{masry-etal-2022-chartqa},
    AI2D~\cite{kembhavi2016diagram},
    GRiT~\cite{peng2023kosmos2},
    VisualGenome~\cite{krishna2017visual},
    RefCOCO/+/g~\cite{kazemzadeh2014referitgame,mao2016generation},
    Synthetic OCR data,
    Common Crawl PDF~\cite{ccpdf}
\end{itemize}


\paragraph*{mPLUG-Owl}~\cite{ye2023mplug}
\begin{itemize}
    \item LLM:\@ LLaMA-7b~\cite{touvron2023llama}
    \item Image Encoder: CLIP ViT-L/14~\cite{radford2021learning}
    \item Vision-Language Connector: Cross-attention and learnt visual queries
    \item Pretraining Data:
    LAION-400M~\cite{schuhmann2021laion},
    COYO-700M~\cite{kakaobrain2022coyo-700m},
    CC3M~\cite{sharma2018conceptual} and
    COCO Captions~\cite{fang2015captions}
    \item Finetuning Data:
    LLaVA~\cite{liu2023visual},
    Alpaca~\cite{alpaca},
    Vicuna~\cite{chiang2023vicuna}
    and Baize~\cite{xu2023baize}
\end{itemize}

\paragraph*{LRV-Instruction-v2}~\cite{liu2023aligning} \\
Same as mPLUG-Owl with one modification.
\begin{itemize}
    \item Finetuning Data:
    LRV-Instruction-v2~\cite{liu2023aligning},
    Alpaca~\cite{alpaca},
    Vicuna~\cite{chiang2023vicuna}
    and Baize~\cite{xu2023baize}
\end{itemize}

\paragraph*{LLaVA-v1.3}~\cite{liu2023visual} \\
\begin{itemize}
    \item LLM:\@ Vicuna-v1.3-7b~\cite{chiang2023vicuna}
    \item Image Encoder: CLIP ViT-L/14~\cite{radford2021learning}
    \item Pretraining Data:
    LAION-400M~\cite{schuhmann2021laion},
    CC3M~\cite{sharma2018conceptual} and
    SBU~\cite{NIPS2011_5dd9db5e}
    \item Finetuning Data:
    LLaVA~\cite{liu2023visual}
\end{itemize}

\paragraph*{LLaVA-v1.5}~\cite{liu2023improved} \\
\begin{itemize}
\item LLM:\@ Vicuna-v1.5-7b~\cite{chiang2023vicuna}
\item Image Encoder: CLIP ViT-L/14~\cite{radford2021learning}
\item Pretraining Data:
LAION-400M~\cite{schuhmann2021laion},
CC3M~\cite{sharma2018conceptual} and
SBU~\cite{NIPS2011_5dd9db5e}
\item Finetuning Data:
LLaVA~\cite{liu2023visual},
VQAv2~\cite{antol2015vqa},
GQA~\cite{hudson2019gqa},
TextVQA~\cite{singh2019towards},
OCR-VQA~\cite{8978122}
and VisualGenome~\cite{krishna2017visual}
\end{itemize}

